The simulated performance of GRANDProto300

GRANDProto300 is a 300-antenna prototype array of the envisioned GRAND (Giant Radio Array for Neutrino Detection) project. The goal of GRANDProto300 is to detect radio signals emitted by cosmic ray-induced air showers, with energies ranging from $10^{16.5}$~eV to $10^{18.5}$~eV, which covers the transition region between Galactic and extragalactic sources. We use simulations to optimize the layout of GRANDProto300 and develop a shower reconstruction method. Based on them, we present the performance of GRANDProto300 for cosmic-ray detection, by means of its effective area, angular resolution, and energy resolution.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".


==> authors.tex <==
J.~Alvarez-Muniz$^{1}$,R.~A.~Batista$^{2}$,A.~Benoit-Levy$^{3}$,T.~Bister$^{4, 5}$,J.~Bolmont$^{6}$,M.~Bustamante$^{7}$,D.~Charrier$^{8}$,Y.~Chen$^{9}$,L.~Cheng$^{10}$,S.~Chiche$^{11}$,J.~Colley$^{6}$,P.~Correa$^{6}$,N.~Cucu Laurenciu$^{4}$,Z.~Dai$^{12}$,R.~M.~de Almeida$^{13}$,S.~de Jong$^{4}$,J.~R.~T.~de Mello Neto$^{14}$,K.~D.~de Vries$^{15}$,P.~B.~Denton$^{16}$,V.~Deocoene$^{11}$,K.~Duan$^{9}$,R.~Duan$^{10}$,B.~Duan$^{9}$,R.~Engel$^{17, 18}$,Y.~Fan$^{9}$,K.~Fang$^{19}$,A.~Ferri\`ere$^{20}$,Q.~Gou$^{21}$,J.~Gu$^{10}$,M.~Guelfand$^{6, 11}$,L.~Guelzow$^{17}$,C.~Guepin$^{22, 23}$,J.~Guo$^{9}$,Y.~Guo$^{21}$,V.~Gupta$^{17}$,A.~Haungs$^{17}$,H.~He$^{9}$,E.~Hivon$^{11}$,H.~Hu$^{21}$,X.~Huang$^{9}$,Y.~Huang$^{10}$,T.~Huege$^{24, 17}$,W.~Jiang$^{25}$,R.~Koirala$^{26, 27}$,K.~Kotera$^{28, 11}$,J.~K\"ohler$^{17}$,B.~L.~Lago$^{29}$,S.~Le Coz$^{6}$,F.~Legrand$^{6}$,J.~Lenain$^{6}$,H.~Li$^{25}$,R.~Li$^{25}$,C.~Liu$^{21}$,R.~Liu$^{26, 27}$,W.~Liu$^{21}$,P.~Ma$^{9}$,F.~Magnard$^{11}$,O.~Martineau-Huynh$^{10, 6, 11}$,A.~Mikhno$^{11}$,P.~Mitra$^{30}$,M.~Mostaf\'a$^{31, 32}$,F.~Mottez$^{33}$,J.~Mouette$^{11}$,K.~Murase$^{31, 32}$,V.~Niess$^{34}$,S.~Ogio$^{35}$,F.~Oikonomou$^{36}$,Z.~Ou$^{37}$,T.~Pierog$^{17}$,L.~W.~Piotrowski$^{30}$,P.~Poisvert$^{6}$,S.~Prunet$^{38}$,X.~Qian$^{39}$,O.~M.~Ramirez$^{40}$,M.~Roth$^{17}$,T.~Sako$^{35}$,H.~Schoorlemmer$^{4, 5}$,F.~Schussler$^{20}$,B.~Steeman$^{4}$,D.~Sz\'alas-Motesiczky$^{4}$,S.~S{\l}awi\'nski$^{30}$,A.~Timmermans$^{15, 4}$,C.~Timmermans$^{4, 5}$,M.~Tueros$^{41}$,S.~Wang$^{9}$,X.~Wang$^{26, 27}$,X.~Wang$^{25}$,X.~Wang$^{39}$,R.~Wang$^{25}$,C.~Watanabe$^{14}$,D.~Wei$^{9}$,F.~Wei$^{25}$,X.~Wu$^{10, 42}$,X.~Wu$^{43}$,X.~Xu$^{25}$,X.~Xu$^{9}$,L.~Yang$^{37}$,X.~Yang$^{9}$,Q.~Yuan$^{9}$,P.~Zarka$^{44}$,H.~Zeng$^{9}$,C.~Zhang$^{45, 46, 17}$,J.~Zhang$^{10}$,K.~Zhang$^{9}$,P.~Zhang$^{25}$,S.~Zhang$^{43}$,H.~Zhang$^{25}$,H.~Zhou$^{47}$
\newline
$^{1}$Departamento de Fisica de Particulas \& Instituto Galego de Fisica de Altas Enerxias, Universidad de Santiago de Compostela, 15782 Santiago de Compostela, Spain$^{2}$Instituto de F{\'\i}sica Te\'orica, Universidad Aut\'onoma de Madrid - CSIC, 28049 Madrid, Spain$^{3}$CEA List, Universit\'e Paris-Saclay,  F-91120 Palaiseau, France$^{4}$Institute for Mathematics, Astrophysics and Particle Physics, Radboud Universiteit, Nijmegen, Netherlands$^{5}$Nationaal Instituut voor Kernfysica en Hoge Energie Fysica, $^{6}$Universite Paris Diderot, Sorbonne Paris Cite, CNRS Laboratoire de Physique Nucleaire et de Hautes Energies, 4 place Jussieu F-75252, Paris Cedex 5, France$^{7}$Niels Bohr International Academy, Niels Bohr Institute, University of Copenhagen, 2100 Copenhagen, Denmark$^{8}$SUBATECH, Institut Mines-Telecom Atlantique, CNRS/IN2P3, Universite de Nantes, Nantes, France$^{9}$Key Laboratory of Dark Matter and Space Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China$^{10}$National Astronomical Observatories, Chinese Academy of Sciences, Beijing 100101, China$^{11}$ Institut d'Astrophysique de Paris, CNRS  UMR 7095, Sorbonne Universite, 98 bis bd Arago 75014, Paris, France$^{12}$University of Science and Technology of China, 230026 Hefei  Anhui, China$^{13}$Universidade Federal Fluminense, EEIMVR Volta Redonda RJ, Brazil$^{14}$Instituto de Fisica, Universidade Federal do Rio de Janeiro, $^{15}$IIHE/ELEM, Vrije Universiteit Brussel, Pleinlaan 2, 1050 Brussels, Belgium$^{16}$High Energy Theory Group, Physics Department Brookhaven National Laboratory, Upton, NY 11973, USA$^{17}$Institute for Astroparticle Physics, Karlsruhe Institute of Technology, D-76021 Karlsruhe, Germany$^{18}$Institute of Experimental Particle Physics, Karlsruhe Institute of Technology, D-76021 Karlsruhe, Germany$^{19}$Wisconsin IceCube Particle Astrophysics Center and Deptartment of Physics, University of Wisconsin-Madison, Madison, WI 53703, USA$^{20}$IRFU, CEA Universite Paris-Saclay, F-91191 Gif-sur-Yvette, France$^{21}$Institute of High Energy Physics, Chinese Academy of Sciences, 19B YuquanLu, Beijing 100049, China$^{22}$Department of Astronomy, University of Maryland, College Park, MD 20742-2421, USA$^{23}$Joint Space-Science Institute, College Park, MD 20742-2421, USA$^{24}$Astrophysical Institute, Vrije Universiteit Brussel, Pleinlaan 2, 1050 Brussels, Belgium$^{25}$Key Laboratory of Antennas and Microwave Technology, Xidian University, Xi{\textquoteright}an 710071, China$^{26}$School of Astronomy and Space Science, Nanjing University, Xianlin Road 163, Nanjing 210023, China$^{27}$Key laboratory of Modern Astronomy and Astrophysics, Nanjing University, Ministry of Education, Nanjing 210023, China$^{28}$Vrije Universiteit Brussel, Pleinlaan 2, B-1050 Brussels, Belgium$^{29}$Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil$^{30}$Faculty of Physics, University of Warsaw, Pasteura 5, 02-093 Warsaw, Poland$^{31}$Department of Astronomy \& Astrophysics, Pennsylvania State University, University Park, PA 16802, USA$^{32}$Center for Multimessenger Astrophysics, Pennsylvania State University, University Park, PA 16802, USA$^{33}$LUTH, Obs. de Paris CNRS Universite Paris Diderot, PSL Research University, 5 place Jules Janssen 92190, Meudon, France$^{34}$CNRS/IN2P3 LPC, Universit\'e Clermont Auvergne, F-63000 Clermont-Ferrand, France$^{35}$Institute for Cosmic Ray Research, University of Tokyo, 5 Chome-1-5 Kashiwanoha, Kashiwa, Chiba 277-0882, Japan$^{36}$Institutt for fysikk, NTNU, Trondheim, Norway$^{37}$School of Physics and Astronomy, Sun Yat-sen University, Zhuhai 519082, China$^{38}$Laboratoire Lagrange, Observatoire de la C\^ote d{\textquoteright}Azur, Universite C\^ote d'Azur, CNRS, Parc Valrose 06104, Nice Cedex 2, France$^{39}$Department of Mechanical and Electrical Engineering, Shandong Management University,  Jinan 250357, China$^{40}$Gravitation Astroparticle Physics Amsterdam, Univesity of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands$^{41}$Instituto de Fisica La Plata, CONICET  Boulevard 120 y 63 (1900)  La Plata$^{42}$Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, China$^{43}$Purple Mountain Observatory, Chinese Academy of Sciences, Nanjing 210023, China$^{44}$LESIA, Observatoire de Paris, CNRS, PSL/SU/UPD/SPC, Place J. Janssen 92195, Meudon, France$^{45}$Kavli Institute for Astronomy and Astrophysics, Peking University, Beijing 100871, China$^{46}$Department of Astronomy, School of Physics, Peking University, Beijing 100871, China$^{47}$Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China

